$\textbf{PLUM}$: Improving Code LMs with Execution-Guided On-Policy Preference Learning Driven By Synthetic Test Cases

Preference learning provides a promising solution to address the limitations of supervised fine-tuning (SFT) for code language models, where the model is not explicitly trained to differentiate between correct and incorrect code. Recent findings demonstrate that on-policy data is the key to successful preference learning, where the preference data is collected using the same policy LM being trained. Inspired by this, we propose PLUM, an on-policy $\textbf{P}$reference $\textbf{L}$earning framework A$\textbf{u}$gmented with test cases for code L$\textbf{M}$ s. The framework operates in three key stages: (1) automatic generation of test cases from natural language instructions, (2) creation of a preference data by evaluating candidate code solutions sampled from the policy, which can then be used to (3) train the policy LM. PLUM levitates the need to train reward models, allowing for large scale on-policy and online preference data collation. PLUM is evaluated on both standard benchmarks (HumanEval, MBPP) and more challenging ones (LiveCodeBench), delivering substantial improvements over original SFT'ed models and other execution-feedback-driven approaches. We show PLUM's benefits are consistent across various widely-used code LMs even they have been well-trained with SFT. For example, PLUM increases pass rates by up to 4.8% on average on standard benchmarks and 11.8% on LiveCodeBench, demonstrating its effectiveness and generalizability. We also demonstrate the benefits of on-policy and online preference learning by comprehensive experimentation.

==> packages.tex <==

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors
%\usepackage{etex}  % fixes ``No room for a new \dimen...'' error from too many packages.
\usepackage{standalone}
\usepackage{latexsym}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{subcaption}
\usepackage{array}
\usepackage{tabu}
\usepackage{makecell}
\usepackage{paralist}
\usepackage{cases}
\usepackage{diagbox}
\usepackage{enumitem}
\usepackage{soul}
\usepackage{multirow}
\usepackage{verbatim}
\usepackage{tabulary}
\usepackage{booktabs}
\usepackage{tabularx}
\usepackage[mathscr]{euscript}
\usepackage{mathtools}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{stmaryrd}
\usepackage{tikz-dependency}
\usetikzlibrary{automata,decorations.markings,arrows,positioning,matrix,calc,patterns,angles,quotes,calc}
\usepackage{adjustbox}
\usepackage{tabularx}
\usepackage{xspace}
\usepackage{tabulary}
\usepackage{afterpage}
\usepackage{bm}
\usepackage{color}
\usepackage{graphicx}
\usepackage{slashbox}
\usepackage[toc,page]{appendix}
\usepackage{makecell}
\usepackage{boldline}
\usepackage[shortcuts]{extdash}  % for non-breaking hyphens. Stack Overflow says it's important for this to be the last package loaded.

\usepackage{blindtext}
\usepackage{graphicx}
\usepackage{capt-of}
\usepackage{booktabs}
\usepackage{varwidth}
\usepackage{pifont}% http://ctan.org/pkg/pifont
\usepackage{wrapfig}

\usepackage[utf8]{inputenc}

% Default fixed font does not support bold face
\DeclareFixedFont{\ttb}{T1}{txtt}{bx}{n}{12} % for bold
\DeclareFixedFont{\ttm}{T1}{txtt}{m}{n}{12}  % for normal

% Custom colors
\usepackage{color}
\definecolor{deepblue}{rgb}{0,0,0.5}
\definecolor{deepred}{rgb}{0.6,0,0}
\definecolor{deepgreen}{rgb}{0,0.5,0}

\usepackage{listings}

% Python style for highlighting
\usepackage{tcolorbox}
% \tcbuselibrary{minted,breakable,xparse,skins}
\tcbuselibrary{breakable,xparse,skins}
\definecolor{bg}{gray}{0.95}
% \DeclareTCBListing{mintedbox}{O{}m!O{}}{%
%   breakable=true,
%   listing engine=minted,
%   listing only,
%   minted language=#2,
%   minted style=default,
%   minted options={%
%     linenos,
%     gobble=0,
%     breaklines=true,
%     breakafter=,,
%     fontsize=\small,
%     numbersep=8pt,
%     #1},
%   boxsep=0pt,
%   left skip=0pt,
%   right skip=0pt,
%   left=25pt,
%   right=0pt,
%   top=3pt,
%   bottom=3pt,
%   arc=5pt,
%   leftrule=0pt,
%   rightrule=0pt,
%   bottomrule=2pt,
%   toprule=2pt,
%   colback=bg,
%   colframe=orange!70,
%   enhanced,
%   overlay={%
%     \begin{tcbclipinterior}
%     \fill[orange!20!white] (frame.south west) rectangle ([xshift=20pt]frame.north west);
%     \end{tcbclipinterior}},
%   #3}


% \setlength{\parindent}{0pt}
% \setlength{\parskip}{0em}
\makeatletter
\newcommand*{\sectionbookmark}[1][]{%
  \bookmark[%
    level=section,%
    dest=\@currentHref,%
    #1%
  ]%
}
\makeatother

\usepackage{abstract}
\setlength{\absleftindent}{0.5in}
\setlength{\absrightindent}{0.5in}

\providecommand{\keywords}[1]
{
  \textbf{\textit{Key words: }} #1
}


==> tables/DPO.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage{colortbl}
% % \usepackage{makecell}

% \begin{table}[]
% \centering
% \begin{tabular}{llrrrrrrr}
% \toprule
% \textbf{Model} &
%   \textbf{Objective} &
%   \textbf{MBPP} &
%   \textbf{MBPP+} &
%   \textbf{HE} &
%   \textbf{HE+} &
%   \textbf{\makecell{Avg. \\ (Base)}} &
%   \textbf{\makecell{Avg. \\ (+)}} &
%   \textbf{\makecell{Avg. \\ (All)}} \\ \midrule
% \multirow{3}{*}{\textbf{MagiCoder-DS-6.7B}}   & \textbf{Baseline} & 75.4 & 61.9 & 66.5 & 60.4 & 71.0          & 61.2          & 66.1          \\
%                                      & \textbf{DPO}      & 75.9 & 63.4 & 65.2 & 61.0 & 70.6          & 67.0          & 66.4          \\
% \rowcolor{cyan!20}                   & \textbf{KTO}      & 79.6 & 66.7 & 71.3 & 65.9 & \textbf{75.5} & \textbf{71.1} & \textbf{75.9} \\ \midrule
% \multirow{3}{*}{\textbf{MagiCoder-S-CL-7B}}   & \textbf{Baseline} & 68.4 & 56.6 & 70.7 & 66.5 & 69.6          & 61.6          & 65.6          \\
%                                      & \textbf{DPO}      & 68.9 & 55.9 & 67.1 & 59.1 & 68.0          & 57.5          & 62.8          \\
% \rowcolor{cyan!20}                   & \textbf{KTO}      & 71.4 & 60.8 & 73.8 & 69.5 & \textbf{72.6} & \textbf{65.2} & \textbf{68.9} \\ \midrule
% \multirow{3}{*}{\textbf{MagiCoder-S-DS-6.7B}} & \textbf{Baseline} & 75.7 & 64.4 & 76.8 & 70.7 & 76.3          & 70.3          & 71.9          \\
%                                      & \textbf{DPO}      & 76.2 & 64.7 & 78.7 & 73.8 & 77.5          & 71.1          & 73.4          \\
% \rowcolor{cyan!20}                   & \textbf{KTO}      & 80.4 & 69.3 & 80.5 & 73.8 & \textbf{80.5} & \textbf{74.9} & \textbf{76.0} \\ \bottomrule
% \end{tabular}
% \caption{Results vs. Training Objectives For Base Models.}
% \label{tab:dpo}
% \end{table}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{colortbl}
% \usepackage{makecell}
% \usepackage{xcolor}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{colortbl}
% \usepackage{makecell}
% \usepackage{xcolor}
% \usepackage{ulem}

\begin{table}[]
\centering
\adjustbox{max width=\textwidth}{
\begin{tabular}{llrrrrrrr}
\toprule
\textbf{Model} &
  \textbf{Objective} &
  \textbf{MBPP} &
  \textbf{MBPP+} &
  \textbf{HE} &
  \textbf{HE+} &
  \textbf{\makecell{Avg. \\ (Base)}} &
  \textbf{\makecell{Avg. \\ (+)}} &
  \textbf{\makecell{Avg. \\ (All)}} \\ \midrule
\multirow{3}{*}{\textbf{MagiCoder-DS-6.7B}}   & \textbf{Baseline} & 75.4 & 61.9 & 66.5 & 60.4 & 71.0          & 61.2          & 66.1          \\
                                     & \textbf{DPO}      & 75.9 & 63.4 & \textcolor{red}{\underline{65.2}} & 61.0 & \textcolor{red}{\underline{70.6}} & 67.0          & 66.4          \\
\rowcolor{cyan!20}                   & \textbf{KTO}      & 79.6 & 66.7 & 71.3 & 65.9 & \textbf{75.5} & \textbf{71.1} & \textbf{75.9} \\ \midrule
\multirow{3}{*}{\textbf{MagiCoder-S-CL-7B}}   & \textbf{Baseline} & 68.4 & 56.6 & 70.7 & 66.5 & 69.6          & 61.6          & 65.6          \\
                                     & \textbf{DPO}     & 68.9 & \textcolor{red}{\underline{55.9}} & \textcolor{red}{\underline{67.1}} & \textcolor{red}{\underline{59.1}} & \textcolor{red}{\underline{68.0}} & \textcolor{red}{\underline{57.5}} & \textcolor{red}{\underline{62.8}} \\
\rowcolor{cyan!20}                   & \textbf{KTO}      & 71.4 & 60.8 & 73.8 & 69.5 & \textbf{72.6} & \textbf{65.2} & \textbf{68.9} \\ \midrule
\multirow{3}{*}{\textbf{MagiCoder-S-DS-6.7B}} & \textbf{Baseline} & 75.7 & 64.4 & 76.8 & 70.7 & 76.3          & 70.3          & 71.9          \\
                                     & \textbf{DPO}      & 76.2 & 64.7 & 78.7 & 73.8 & 77.5          & 71.1          & 73.4          \\
\rowcolor{cyan!20}                   & \textbf{KTO}      & 80.4 & 69.3 & 80.5 & 73.8 & \textbf{80.5} & \textbf{74.9} & \textbf{76.0} \\ \bottomrule
\end{tabular}}
\caption{KTO vs. DPO when used with \name to train SFT-ed models (\textbf{Baseline}). 
\textcolor{red}{\underline{Red underlined numbers}} indicate performance that are worse than the baseline's.}
\label{tab:dpo}
\end{table}

